Diagonally-Addressed Matrix Nicknack: How to improve SpMV performance

We suggest a technique to reduce the storage size of sparse matrices at no loss of information. We call this technique Diagonally-Adressed (DA) storage. It exploits the typically low matrix bandwidth of matrices arising in applications. For memory-bound algorithms, this traffic reduction has direct benefits for both uni-precision and multi-precision algorithms. In particular, we demonstrate how to apply DA storage to the Compressed Sparse Rows (CSR) format and compare the performance in computing the Sparse Matrix Vector (SpMV) product, which is a basic building block of many iterative algorithms. We investigate 1367 matrices from the SuiteSparse Matrix Collection fitting into the CSR format using signed 32 bit indices. More than 95% of these matrices fit into the DA-CSR format using 16 bit column indices, potentially after Reverse Cuthill-McKee (RCM) reordering. Using IEEE 754 double precision scalars, we observe a performance uplift of 11% (single-threaded) or 17.5% (multithreaded) on average when the traffic exceeds the size of the last-level CPU cache. The predicted uplift in this scenario is 20%. For traffic within the CPU's combined level 2 and level 3 caches, the multithreaded performance uplift is over 40% for a few test matrices.

==> preamble/abbreviations.tex <==
\newcommand\eg{e.g\@.} % exampli gratia
\newcommand\ie{i.e\@.} % id est
\newcommand\cf{cf\@.} % confer/conferatur

\newcommand\ao{a.o\@.} % among others
\newcommand\wrt{w.r.t\@.} % with respect to


==> preamble/acronym.tex <==
\usepackage{acronym}

\newacro{DA}{Diagonally-Adressed}
\newacro{DA-CSR}{Diagonally-Adressed \ac{CSR}}
\newacro{BSR}{Block \ac{CSR}}
\newacro{COO}{Coordinate}
\newacro{CSC}{Compressed Sparse Columns}
\newacro{CSR}{Compressed Sparse Rows}
\newacro{MKL}{Math Kernel Library}
\newacro{SpMV}{Sparse Matrix Vector}
\newacro{SpMM}{Sparse Matrix Matrix}
\newacro{RSB}{Recursive Sparse Blocks}
\newacro{RCM}{Reverse Cuthill-McKee}


==> preamble/colors.tex <==
\definecolor{ovgu}     {RGB}{122,   0,  63}
\definecolor{ovgu math}{RGB}{209,  63,  88}
\definecolor{ovgu nat} {RGB}{  5, 165,  53}
\definecolor{ovgu eit} {RGB}{148, 193,  45}
\definecolor{ovgu hw}  {RGB}{243, 145,   0}
\definecolor{ovgu vst} {RGB}{148,  22, 128}
\definecolor{ovgu med} {RGB}{  0,  45,  92}
\definecolor{ovgu inf} {RGB}{  0, 104, 180}
\definecolor{ovgu mb}  {RGB}{  0, 158, 227}
\definecolor{ovgu ww}  {RGB}{ 93, 142, 166}
\definecolor{ovgu hw}  {RGB}{243, 145,   0}

\colorlet{rainbow1}{ovgu}
\colorlet{rainbow2}{ovgu inf}
\colorlet{rainbow3}{ovgu eit}
\colorlet{rainbow4}{ovgu hw}
\colorlet{rainbow5}{ovgu math}


==> preamble/listings.tex <==
\usepackage{listings}

\lstset{
basicstyle=\ttfamily,
commentstyle=\color{gray},
%keywordstyle=\bfseries,
%stringstyle=\ttfamily,
showstringspaces=false,
numbers=none,
language=C++,
%keepspaces=true,
%columns=fixed,
moredelim=**[is][{\usebeamercolor[fg]{structure}}]{|}{|},
numbers=left,
numbersep=1ex,
numberstyle={\scriptsize\color{gray}},
morekeywords={int8_t,int16_t,int32_t,int64_t,oindex_t,iindex_t,scalar_t},
}

\newcommand\oindext{\lstinline!oindex_t!}
\newcommand\iindext{\lstinline!iindex_t!}
\newcommand\scalart{\lstinline!scalar_t!}

\newcommand\oindexs{\lstinline!sizeof(oindex_t)!}
\newcommand\iindexs{\lstinline!sizeof(iindex_t)!}
\newcommand\scalars{\lstinline!sizeof(scalar_t)!}

\newcommand\xshift{\lstinline!xshift!} % variable in snippets/dacsr_spmv.c


==> preamble/misc.tex <==
% props to https://tex.stackexchange.com/a/98011/95100
\DeclareMathAlphabet{\mathup}{OT1}{\familydefault}{m}{n}

\newcommand\nnz{\ensuremath{\mathup{nnz}}}
\newcommand\ncols{\ensuremath{\mathup{ncols}}}
\newcommand\nrows{\ensuremath{\mathup{nrows}}}
\newcommand\runtime{t}
\newcommand\perf{P} % power
\newcommand\eff{\eta} % efficiency
\newcommand\traffic{\text{traffic}} % Q; same as heat [J] and electric charge [C]
\newcommand\baseline{_\text{baseline}}
\newcommand\candidate{_\text{candidate}}
\newcommand\ideal{_\text{ideal}}

\newcommand\F{\mathbb F} % arbitrary field
\newcommand\R{\mathbb R} % real numbers
\newcommand\Z{\mathbb Z} % integer numbers
\newcommand\N{\mathbb N} % natural numbers

\newcommand\rowptr{\ensuremath{\mathup{rowptr}}}
\newcommand\colids{\ensuremath{\mathup{colids}}}
\newcommand\values{\ensuremath{\mathup{values}}}

